A Decomposition and Metric-Based Evaluation Framework for Microservices

Migrating from monolithic systems into microservice is a very complex task. Companies are commonly decomposing the monolithic system manually, analyzing dependencies of the monolith and then assessing different decomposition options. The goal of our work is two-folded: 1) we provide a microservice measurement framework to objectively evaluate and compare the quality of microservices-based systems; 2) we propose a decomposition system based on business process mining. The microservice measurement framework can be applied independently from the decomposition process adopted, but is also useful to continuously evaluate the architectural evolution of a system. Results show that the decomposition framework helps companies to easily identify the different decomposition options. The measurement framework can help to decrease the subjectivity of the decision between different decomposition options and to evaluate architectural erosion in existing systems.

==> 04Validation.tex <==
\kari{TODO: check and comment: SERVER-side only}

In this section, we validate the decomposition framework proposed in Section III. With this study, we aim to understand whether our approach can support developers in easily identifying different slicing options. For this purpose, we performed an industrial case study to compare the ad-hoc decomposition solution proposed by the software architect with the solutions proposed by our approach. 



According to our expectations, we formulated the goal of the case study  as: 

\noindent \textit{Analyze} the proposed decomposition solutions \\
\noindent \textit{for the purpose of} evaluating and comparing \\ 
\noindent \textit{with respect to} the perceived slicing easiness and usefulness \\
\noindent \textit{in the context of} the migration of a monolithic system to microservices\\
\noindent \textit{from the point of view of} software architects.\\


We formulated the questions of the case study as follows and further derived questions and metrics from them: 






% According to our expectations, we formulated the questions of the case study as follows and further derived questions and metrics from them: 

\vspace{2mm}
\begin{tabular}
{@{}p{1.0cm}p{9cm}@{}}
\textbf{RQ1} & Q1:	Does adopting the proposed decomposition framework \textbf{ease} the identification of different microservices?   \\
\textbf{RQ2} & Q2:	What do the developers, software architects, and project manager think about the \textbf{applicability} of this approach?  \\
\textbf{RQ3} & Q3:	Are the developers willing to \textbf{use} the approach in the future? \\
\end{tabular}
\vspace{2mm}

We answered our questions by surveying the project manager and the software architect who first manually applied the decomposition process as usual and then evaluate the decomposition options proposed by our framework. The measures identified for the questions were derived from the Technology Acceptance Model ~\cite{Venkatesh00}. All questions were evaluated based on a 5-point ordinal Likert scale with the following options: 1 = strongly disagree, 2 = disagree, 3 = neither agree nor disagree, 4 = agree, 5 = strongly agree. 

\textbf{Q1 – Perceived ease of use:} Here we aim to compare the perceived easiness of our approach with that of the experience-based (ad-hoc) approach. We adopted the Technology Acceptance Model ~\cite{Venkatesh00} to collect measures about the ease of use of our approach, identifying the following metrics: 
\begin{itemize}
    \item The process-mining approach would be easy for me to use during the decomposition phase.
    \item It would be easy for me to become skillful at using the process-mining approach to decompose a monolithic system.
\end{itemize}

\textbf{Q2 - Applicability:} What do the participants think about the applicability of our approach? To answer this question, we collected the time overhead needed to perform the process-mining approach.
Perceived usefulness: measures the degree to which the participants considered the approach useful for making project decisions. The evaluated criteria were:
\begin{itemize}
    \item I am sure that I was able to better decompose the system with this approach.
    \item I was able to find alternative decomposition strategies.
    \item I was able to better decompose the system, but the time required with the new approach is too much compared to its benefits.
    \item I was able to better decompose the system, but the effort needed to trace the information on the log file is too much compared to the benefits of the approach.
    \item The approach helped me to understand existing architectural issues in the existing monolithic system
\end{itemize}

\textbf{Perceived understandability:} measures the effort needed by the subject to understand the approach built or whether the participants will need to exert little effort to understand the relationship with the system concepts.
\begin{itemize}
\item It was easy for me to understand how the approach works.
Perceived easiness: measures the degree to which the subject believed that he or she was able to make project decisions easier than without the approach.
\item It was easy for me to identify decomposition options with the support of this approach.
\item I was able to identify decomposition options with less effort compared to the ad-hoc manual decomposition. 
\item I was able to identify decomposition options more accurately.
\end{itemize}

\textbf{Self-efficacy by applying the technique:} The perceived ability to decompose a monolithic system into microservices by means of our proposed approach. 
\begin{itemize}
    \item It was easy for me to keep an overview of the project and of the different decomposition options.
    \item The approach helped me to increase the quality of the decompositions.
\end{itemize}

\textbf{Q3 - Willingness to use our approach in the future:} With this question, we aim to understand whether the company would be willing to use our system in the future. We collected this measure with the following question:
\begin{itemize}
    \item I will adopt this approach in the future. 
\end{itemize}


Table~\ref{tbl:excel-table} report the list of questions and the results of this study.

\begin{table*}
  \includegraphics[trim={2cm 5cm 2cm 15.2cm},clip,width=\textwidth]{Figures/BigTable.pdf}
    \caption{The Questionnaire adopted in this study - Results (From~\cite{DavideKari2019})}
  \label{tbl:excel-table}
\end{table*}

\subsection{Study Context }
The approach was applied in an SME in Milan (Italy). The company develops a document management system for bookkeeping, for Italian tax accountants. The goal of the system is to make it possible to manage the whole bookkeeping process, including management of the digital invoices, sending the invoice to the Ministry of Economic Development, and fulfilling all the legal requirements, which usually change every year. 

The system is developed by two teams of 4 developers, plus two part-time developers following the moonlight scrum process~\cite{TaibiMoonlight}, the software architect and a project manager.  currently being used by more than 2000 tax accountants, who need to store more than 20M invoices per year. The system has been developed for more than 12 years and is now composed of more than 1000 Java classes. 

The Italian government usually updates the bookkeeping process between December and January of every year, which involves not only changing the tax rate but also modifying the process of storing the invoices. However, tax declarations can be made starting in March/April of each year. Therefore, in the best case, the company has between two to four months to adapt their software to the new rules in order to enable tax accountants to work with the updated regulations from March/April. 


Up to now, the company used to hire a consultancy company to help them during these three months of fast-paced work. However, since the system is growing year after year, they decided to migrate to microservice to facilitate maintenance of the system~\cite{Nyyti19} and to distribute the work to independent groups, reducing communication needs and supporting fast delivery~\cite{TaibiRequirements}\cite{TaibiCommunication}.

\subsection{Study Execution}
We performed this study in three steps: 

\vspace{2mm}
\begin{tabular}
{@{}p{1cm}p{10.5cm}@{}}
\textbf{Step 1} & 
% Q1: 
The software architect manually identified the different microservices and a decomposition strategy.   \\
\textbf{Step 2} & 
% Q2: 
We applied our 6-steps process to identify different decomposition solutions and then we compared them to the solution proposed by the software architect.   \\
\textbf{Step 3} & 
% Q3: 
The software architect and the project manager provided feedback on the usefulness of our approach.
\end{tabular}
\vspace{2mm}

\subsection{Case Study Results}
With the support of the development team, the software architect manually identified a set of microservices. He first drew the dependency graph with Structure 101.  

Then we applied our approach to mine their log files. The company already logged all the operations of their systems with Log4J\footnote{https://logging.apache.org/log4j}, tracing all the information reported in Table~\ref{tab:Freq}, together with other information such as the user involved in the process, the ID of the customer with which the tax accountant is currently working, and other information related to the current invoices. 

From this information, we identified 39 different business processes with DISCO. For confidentiality reasons, we can only disclose a high-level and anonymized portion of the system. Figure~\ref{fig:Fig4} depicts an example of two business processes (save invoice and view invoice). We then calculated the frequency of each process. DISCO can automatically draw thicker arcs between processes, thereby simplifying the approach.  

Of 39 processes, three processes had been used only three times during one year of logging, 17 processes less than 1000 times, and 12 processes between 1000 and 10K times; five processes had been used more than 60B times. This distribution was initially expected for most of the processes. The most frequently used processes were due to the submission of the invoices from each tax accountant. 


% \begin{table*}[]
% \small\centering
% \begin{tabular}{p{2cm}p{1.5cm}|p{7cm}|p{1.5cm}|p{1.5cm}}\\ \hline 
% \multicolumn{2}{c|}{Questions} & Metrics & Project Manager & Software Architect \\ \hline
% \multirow{2}{*}{Q1 – Perceived ease of use} & & The proposed approach would be easy for me to use in the decomposition phase & 4 & 5 \\ 
% & & It would be easy for me to become skillful at using the process-mining approach to decompose a monolithic system & 3 & 4 \\ \hline
% Applicability  & & I am sure that I was able to better decompose the system with this approach & 5 & 5 \\
% Perceived usefulness & & I was able to find alternative decomposition strategies & 5 & 5 \\



% \end{tabular}
% \caption{The Questionnaire adopted in this study - Results}
% \label{tab:Results}
% \end{table*}
% trim={<left> <lower> <right> <upper>}
% \begin{figure*} []
%     \centering
%     \includegraphics[trim={2cm 5cm 2cm 15.2cm},clip,width=\textwidth]{Figures/BigTable.pdf}
%     \captionof{Table}{The Questionnaire adopted in this study - Results}
%     \label{Table:XXX}
% \end{figure*}

\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{p{0.6cm}|p{0.8cm}|p{0.8cm}|p{0.95cm}|p{0.8cm}|p{0.6cm}|p{0.8cm}|p{0.9cm}|p{0.8cm}|p{0.6cm}|p{0.8cm}|p{0.9cm}|p{0.8cm}}  \hline 
\multirow{3}{*}{MS} & \multicolumn{12}{c}{Decomposition Solutions} \\ \cline{2-13}
& \multicolumn{4}{c}{Solution 1} & \multicolumn{4}{|c}{Solution 2} & \multicolumn{4}{|c}{Solution 3} \\ \cline{2-13}
 & CBM	&\#Links	&\#Classes	&\#Dupl. Classes&	CBM	&\#Links	&\#Classes&	\#Dupl. Classes	&CBM	&\#Links&	\#Classes &	\#Dupl. Classes \\ \hline
MS1&	0.08&	6&	75	&2&	0.26&	7&	27	&0	&0.13&	5&	39	&2 \\
MS2&	0.29&	9&	31	&4	&0.33&	11&	33	&2	&0.26&	7&	27&	0 \\
MS3	&0.08&	2&	25&	0	&0.06&	2	&33	&1	&0.33&	10	&31	&4 \\
MS4&	0.16&	7&	43	&2	&0.08&	4	&50	&3	&0.17	&7	&41	&3 \\
MS5	&0.17&	5	&30	&0	&0.18&	10&	56&	0	&0.14	&4	&28&	0 \\ 
\hline 
\end{tabular}
\caption{Decomposition metrics for the decomposition options}
\label{tab:DecompositionMetrics}
\end{table*}



\begin{figure} []
    \centering
    \includegraphics[width=0.6\columnwidth]{Figures/Fig4.pdf}
    \caption{The Proposed Slicing Options – (Simplified example) (From~\cite{DavideKari2019})}
    \label{fig:Fig4}
\end{figure}

Based on the previous step, the software architect, together with the project manager, identified three slicing options, taking care to avoid circular dependencies between services, especially in the case of the three classes that suffered from an existing circular dependency. Therefore, we proceeded with the calculation of cohesion and coupling of the different slicing options. The CBM was counted from the outgoing calls reported in the output of DISCO tool.

The first solution was composed of 25 microservices (19 classes duplicated) with an average CBM of 0.16; the second solution was composed of 27 microservices (21 classes duplicated) with an average CBM of 0.16; while the third solution was composed of 21 microservices (14 classes duplicated) with an average CBM of 0.22. Table~\ref{tab:DecompositionMetrics} shows the measures collected for five microservices of each decomposition solution. 

The first initial result is the list of classes, methods, and database tables used in the different processes together with their frequency of usage. Moreover, the solution proposed by the software architect had higher coupling and was more complex than the ones identified with the process-mining approach. The analysis of log files also shows that some processes were used much more than expected while one process traverses an unexpected set of classes performing an incorrect process. Moreover, they also discovered three unexpected circular dependencies and the presence of two harmful code smells~\cite{TaibiJL17}.

One of the most important decision drivers that lead to the selection of one of the three identified solutions, was the type of decomposition. One of the selected decomposition options proposed to slice the system based on the need of creating more shared libraries. Shared libraries commonly increase the complexity of the migration, and increase the maintenance complexity. The other reason was related to the developer’s knowledge and the code ownership. The selected solution allowed to split the systems reducing the need of re-organizing the teams and re-allocating the responsibility of the code. The developers preferred to migrate the code they have written in the past, instead of migrating the code written by other developers. 

